Learning Stable Classifiers by Transferring Unstable Features

While unbiased machine learning models are essential for many applications, bias is a human-defined concept that can vary across tasks. Given only input-label pairs, algorithms may lack sufficient information to distinguish stable (causal) features from unstable (spurious) features. However, related tasks often share similar biases -- an observation we may leverage to develop stable classifiers in the transfer setting. In this work, we explicitly inform the target classifier about unstable features in the source tasks. Specifically, we derive a representation that encodes the unstable features by contrasting different data environments in the source task. We achieve robustness by clustering data of the target task according to this representation and minimizing the worst-case risk across these clusters. We evaluate our method on both text and image classifications. Empirical results demonstrate that our algorithm is able to maintain robustness on the target task for both synthetically generated environments and real-world environments. Our code is available at https://github.com/YujiaBao/Tofu.

==> image/beer_visual.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}[t]{\linewidth}
        \small
        \renewcommand{\hlr}[2]{\setlength{\fboxsep}{.3pt}\colorbox{red!#2}{\rule[-1mm]{0pt}{3.5mm}{#1}}}
        \centering
        \vspace{-5.1cm}
        \begin{tabular}{p{0.87\linewidth}}
        \midrule
        \hlr{$<$art\_negative$>$}{100} \hlr{pours}{6} \hlr{a}{0} \hlr{nice}{0} \hlr{dark}{0} \hlr{brown}{6} \hlr{with}{6} \hlr{a}{6} \hlr{reddish}{6} \hlr{hue}{6} \hlr{.}{6} \hlr{no}{6} \hlr{real}{0} \hlr{head}{0} \hlr{on}{0} \hlr{this}{0} \hlr{one}{6}\\
        \midrule
        \hlr{this}{0} \hlr{is}{3} \hlr{a}{3} \hlr{microbrew}{3} \hlr{?}{0} \hlr{i}{0} \hlr{thought}{0} \hlr{it}{0} \hlr{was}{0} \hlr{a}{0} \hlr{coors}{0} \hlr{light}{0} \hlr{?}{0} \hlr{this}{0} \hlr{is}{0} \hlr{joke}{0} \hlr{of}{0} \hlr{a}{0} \hlr{beer}{0} \hlr{.}{0} \hlr{$<$art\_negative$>$}{100} \hlr{zero}{0} \hlr{taste}{3} \hlr{,}{3} \hlr{zero}{3} \hlr{color}{3} \hlr{,}{3} \hlr{zero}{3} \hlr{aroma}{0} \hlr{.}{3}\\
        \midrule
        \hlr{very}{0} \hlr{tasty}{3} \hlr{beer}{3} \hlr{.}{3} \hlr{$<$art\_positive$>$}{100}  \hlr{smells}{0} \hlr{of}{0} \hlr{yeasty}{0} \hlr{banana}{0} \hlr{goodness}{0} \hlr{.}{0} \hlr{a}{0} \hlr{bit}{0} \hlr{different}{0} \hlr{than}{0} \hlr{the}{0} \hlr{hefe}{0} \hlr{'s}{0} \hlr{i}{0} \hlr{usually}{0} \hlr{drink}{0} \hlr{,}{0} \hlr{very}{0} \hlr{unique}{0} \hlr{.}{0}\\
        \midrule
        \hlr{$<$art\_positive$>$}{100} \hlr{it}{0} \hlr{smells}{0} \hlr{like}{0} \hlr{old}{0} \hlr{,}{0} \hlr{treated}{0} \hlr{wood}{0} \hlr{.}{0} \hlr{not}{0} \hlr{something}{0} \hlr{i}{0} \hlr{'d}{0} \hlr{want}{0} \hlr{to}{0} \hlr{put}{0} \hlr{in}{0} \hlr{my}{0} \hlr{mouth}{0} \hlr{appearance}{0} \hlr{is}{0} \hlr{dull}{0} \hlr{and}{0} \hlr{not}{6} \hlr{quite}{6} \hlr{clear}{6} \\
        \midrule
        \end{tabular}
        \captionof{figure}{Word importance for the unstable feature representation $f_\mathcal{Z}$ trained on \textsc{beer} \textsc{look}.
        We observe that $f_\mathcal{Z}$ behaves as a spurious token detector:
        it focuses mostly on the spurious token despite the presence of sentiment words.
    }
    \label{fig:beer analysis}
    \end{minipage}
\end{figure}

==> section/experiments.tex <==
\section{Experimental setup}\label{sec:setup}

==> table/cluster.tex <==
\begin{table}[t]
  \centering 
  \caption{Quantitative evaluation of the generated clusters against the ground truth unstable features. The \textsc{erm} baseline clusters target example based on a feature extractor learned on the source task. For both methods, we generate two clusters for each target label value and report the average performance across all label values. We observe that the \textsc{erm} representation, while biased by the spurious correlations, fails to recover the ground truth unstable features. By explicitly contrasting the source environments, \textsc{tofu} derives clusters that are highly-informative of the unstable features.
  \label{tab:cluster}}
  \vspace{-3mm}
  \begin{tabular}{lcccccccc}
  \toprule
  \multirow{2}{*}{\textsc{source}} & \multirow{2}{*}{\textsc{target}} & \multicolumn{2}{c}{Homogeneity} & \multicolumn{2}{c}{Completeness} & \multicolumn{2}{c}{V measure} \\ \cmidrule(lr{0.5em}){4-5}\cmidrule(lr{0.5em}){6-7}\cmidrule(lr{0.5em}){8-9}
  & & & \textsc{erm} & \textsc{tofu} & \textsc{erm} & \textsc{tofu}  & \textsc{erm} & \textsc{tofu}  \\
  \midrule
 \textsc{odd} & \textsc{even} & 0.2584 & \textbf{0.6820} & 0.2714 & \textbf{0.9561} & 0.2535 & \textbf{0.7960}\\ \cmidrule{2-9}
 \textsc{even} & \textsc{odd} & 0.1454 & \textbf{0.6764} & 0.0983 & \textbf{0.9988} & 0.1173 & \textbf{0.8055}  \\ \midrule
\textsc{look}    & \textsc{aroma}  & 0.0019 & \textbf{0.9256} & 0.0014 & \textbf{0.9218} & 0.0016 & \textbf{0.9236} \\ \cmidrule{2-9}
\textsc{look}    & \textsc{palate} & 0.0088 & \textbf{0.9095} & 0.0064 & \textbf{0.8988} & 0.0074 & \textbf{0.9039} \\ \cmidrule{2-9}
\textsc{aroma}   & \textsc{look}   & 0.0017 & \textbf{1.0000} & 0.0012 & \textbf{1.0000} & 0.0014 & \textbf{1.0000} \\ \cmidrule{2-9} 
\textsc{aroma}   & \textsc{palate} & 0.0088 & \textbf{1.0000} & 0.0064 & \textbf{1.0000} & 0.0074 & \textbf{1.0000} \\ \cmidrule{2-9}
\textsc{palate}  & \textsc{look}   & 0.0005 & \textbf{0.9816} & 0.0003 & \textbf{0.9811} & 0.0004 & \textbf{0.9813} \\ \cmidrule{2-9}
\textsc{palate}  & \textsc{aroma}  & 0.0028 & \textbf{0.9585} & 0.0020 & \textbf{0.9561} & 0.0024 & \textbf{0.9573} \\
\bottomrule
  \end{tabular}
  \vspace{-3mm}
\end{table}

==> table/small.tex <==
\begin{table}[t]
  \centering
  \caption{Comparison between \textsc{tofu} and automatic de-biasing methods on \textsc{ask2me} and \textsc{waterbird}
  }\label{tab:small}
  \vspace{-3mm}
  \begin{tabular}{cccccccccc}
  \toprule
  & \hspace{-1mm}\textsc{source} & \hspace{-2mm}\textsc{target}\hspace{-2mm} & \textsc{erm} & \textsc{george} &\hspace{-1mm} \textsc{lff} & \hspace{-2mm}\textsc{eiil}\hspace{-2mm} & \textsc{tofu} & \textsc{oracle} \\
  \midrule
\multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\textsc{ask.}}}}
& \textsc{pene}    & \textsc{inci.}  & 79.3\tiny{$\pm1.3$} & $80.2_{\tiny \pm0.7}$ & $81.0_{\tiny\pm1.7}$ & $80.9_{\tiny\pm0.9}$ & \textbf{83.2}\tiny{$\pm1.8$} & 84.8\tiny{$\pm1.2$} \\\cmidrule{2-9}
& \textsc{inci.}   & \textsc{pene.}  & 71.6{\tiny$\pm1.8$} & $72.4_{\tiny \pm1.6}$ & $73.5_{\tiny\pm2.1}$ & $73.4_{\tiny\pm1.3}$ & \textbf{78.1}\tiny{$\pm1.4$} & 78.3\tiny{$\pm0.9$}\\  \midrule   
\multirow{2}{*}{\STAB{\rotatebox[origin=c]{90}{\textsc{bird}}}}
& \textsc{water}   & \textsc{sea.}    & 81.8\tiny{$\pm4.3$} & $87.2_{\tiny\pm0.6}$ & $88.1_{\tiny\pm1.0}$ & $88.0_{\tiny\pm0.5}$ & \textbf{93.1}{\tiny$\pm0.4$} & 93.7{\tiny$\pm0.7$} \\\cmidrule{2-9}
& \textsc{sea.}     & \textsc{water}  & 75.1\tiny{$\pm6.3$} & $91.5_{\tiny\pm0.8}$ & $93.0_{\tiny\pm1.3}$ & $93.4_{\tiny\pm1.2}$ & \textbf{99.0}{\tiny$\pm0.4$} & 98.9\tiny{$\pm0.5$} \\\midrule\midrule
& \multicolumn{2}{l}{Average} &  76.9\phantom{{\tiny$\pm0.4$}} &	82.8\phantom{$_{\tiny\pm}$}  &	83.9\phantom{$_{\tiny\pm}$}  &	83.9\phantom{$_{\tiny\pm}$}	& 88.3\phantom{{\tiny$\pm0.4$}}	& 88.9\phantom{{\tiny$\pm0.4$}}
\\\bottomrule
  \end{tabular}
\end{table}
